Using hyperelliptic curves to find positive polynomials that are not a sum of three squares in R(x, y)

This article deals with a quantitative aspect of Hilbert's seventeenth problem: producing a collection of real polynomials in two variables of degree 8 in one variable which are positive but are not a sum of three squares of rational fractions. As explained by Huisman and Mahe, a given monic squarefree positive polynomial in two variables x and y of degree in y divisible by 4 is a sum of three squares of rational fractions if and only if the jabobian variety of some hyperelliptic curve (associated to P) has an "antineutral" point. Using this criterium, we follow a method developped by Cassels, Ellison and Pfister to solve our problem : at first we show the Mordell-Weil rank of the jacobian variety J associated to some polynomial is zero (this step is done by doing a 2-descent), and then we check that the jacobian variety J has no antineutral torsion point.

==> 46-Exemples.tex <==
\begin{scoro}
Let $\eta,$ $\omega ,$ and $\rho$ be three real numbers. We assume $\eta,$ $\omega ,$ and $\rho$ to be algebraically independants over $\Q$. Let note 
$$b_{1}=\frac{\rho^{2}-\eta^{2}}{\omega^{2}-\eta^{2}}+\frac{\eta^{2}-\omega^{2}}{4}.$$
We consider two polynomials $B(x):=(x+b_{1})^{2}-\eta^{2}$ et $C(x):=2(x+b_{1})+\omega^{2}-\eta^{2}-1.$  $\omega >1+|\eta |$, $\omega^{2}-\eta^{2}>2\omega $, et $b_{1}>1+\frac{\omega^{2}-\eta^{2}}{2}$. \\

Under those assumptions the polynomial 
$$P(x,y):=\left( y^{2}+1\right)\left( y^{2}+C\left( x^{2}\right)\right)\left( y^{4}+\left( 1+C\left( x^{2}\right)\right) y^{2}+B\left( x^{2}\right)\right)$$
is positive but is not a sum of three squares in $\R (x,y)$.
\end{scoro}

\begin{scoro}
We consider Theorem \ref{theo-final-pas-somme-3-carres-46} with $\eta :=23$ $\omega :=34$, $\rho :=547$. In that case we have
$$\begin{array}{l}
b_{1}=\frac{\rho^{2}-\eta^{2}}{\omega^{2}-\eta^{2}}+\frac{\eta^{2}-\omega^{2}}{4}=\frac{14063}{44},\\$$
\\
B(x):=(x+b_{1})^{2}-\eta^{2}=x^{2}+\frac{14063}{22}x+\frac{196743825}{1936}\textrm{ et }\\
\\
C(x):=2(x+b_{1})+\omega^{2}-\eta^{2}-1=2x+\frac{27835}{22}.\\
\end{array}$$ 

Following Theorem \ref{theo-final-pas-somme-3-carres-46}, the polynomial 
$$P(x,y):=\left( y^{2}+1\right)\left( y^{2}+C\left( x^{2}\right)\right)\left( y^{4}+\left( 1+C\left( x^{2}\right)\right) y^{2}+B\left( x^{2}\right)\right)\in\Q (x,y)$$
is positive but is not a sum of three squares in $\R (x,y)$.
\end{scoro}
